Methods for Efficient Unfolding of Colored Petri Nets

Colored Petri nets offer a compact and user friendly representation of the traditional P/T nets and colored nets with finite color ranges can be unfolded into the underlying P/T nets, however, at the expense of an exponential explosion in size. We present two novel techniques based on static analysis in order to reduce the size of unfolded colored nets. The first method identifies colors that behave equivalently and groups them into equivalence classes, potentially reducing the number of used colors. The second method overapproximates the sets of colors that can appear in places and excludes colors that can never be present in a given place. Both methods are complementary and the combined approach allows us to significantly reduce the size of multiple colored Petri nets from the Model Checking Contest benchmark. We compare the performance of our unfolder with state-of-the-art techniques implemented in the tools MCC, Spike and ITS-Tools, and while our approach is competitive w.r.t. unfolding time, it also outperforms the existing approaches both in the size of unfolded nets as well as in the number of answered model checking queries from the 2021 Model Checking Contest.

==> Introduction/Introduction.tex <==
\section{Introduction} \label{sec:Introduction}
When modelling large systems it is important to verify that the system is working as intended. Since many systems are under constant change it is necessary to automate the verification process. One of the most widely used of such verifiable models are Petri nets introduced by Carl A. Petri in 1962~\cite{CarlPetriNets}. 

Petri nets are most often seen in a classical Place/Transition (P/T) form and thus most verification techniques have been developed for P/T nets~\cite{MurataPaper}. However, P/T nets often become too large and incomprehensible for humans to read. Therefore, colored Petri nets (CPN)~\cite{CPNJensen} have been introduced which are compressed versions of Petri nets, that employ different techniques from programming such as types, variables and logical expressions. 

In CPNs each place is assigned a color domain and each token in that place has a color from the color domain. Arcs have expressions that define what colored tokens to consume and produce and transitions have guard expressions that restrict when a transition may fire. 

A CPN can be translated into a P/T net if every color domain is finite through a process called \textit{unfolding}, which allows the use of efficient verification methods already developed for P/T nets. When unfolding a CPN each place is unfolded into a new place for each color that a token can take in the place; a naive approach is to create a new place for each color in the color domain of the place. Transitions are unfolded such that each binding of variables that satisfies the guard is unfolded into a new transition in the unfolded net. 

The size of an unfolded net can be exponentially larger than the colored net and therefore requires certain optimizations and analyses to unfold in realistic time and memory. Several types of analyses have been proposed that consider especially transition guards and arc expressions~\cite{MCCUnfolder, PatternPaper, IDDUnfolder}.

However, even with the optimizations there still exists CPNs that cannot be unfolded. As an example, the largest instances of the nets \textit{FamilyReunion}~\cite{FamilyReunionNet, FamilyReunionPaper} and \textit{DrinkVendingMachine}~\cite{DrinkVendingMachineNet, DrinkVendingMachinePaper} from the Model Checking Contest~\cite{mcc:2020} have yet to be unfolded. This is the case since the color domains and number of possible bindings are far too large to be unfolded in realistic time and memory with current techniques. Even if the net is unfolded it may still be too large to verify due to the exponential increase in size. 

%In ~\cite{MCCUnfolder} they claim that unfolding these nets will require more memory and computation time and is simply a matter of the hardware not being good enough

We propose two new methods for statically analysing a CPN to reduce the size of the unfolded P/T net. The first method called \textit{color quotienting} uses the fact that sometimes multiple colors behave the same throughout the colored net. If such colors exist in the net we can create equivalence classes that represents the colors with similar behaviour. As such, we can reduce the amount of colors that we need to consider when unfolding, because we now only have to consider the equivalence class of colors instead of each color individually.


The second method called \textit{color approximation} detects which colors may actually be present in any given place s.t. we only unfold places for the colors that can exist. This method also allows for invalidating bindings that are dependent on unreachable colors thus reducing the amount of transitions that are unfolded.  

\paragraph{Related work:}
Several unique approaches for unfolding CPNs effectively have been proposed. In~\cite{PatternPaper} Heiner et al. analyses the arc- and guard expressions to reduce the amount of bindings that need to be considered for a given transition by collecting \textit{patterns}. The pattern analysis is implemented in the tool Snoopy~\cite{SnoopyTool}. The color approximation method captures the reductions of the pattern analysis. In~\cite{IDDUnfolder} the same authors present a technique for representing and using patterns utilizing Interval Decision Diagrams. This technique is used in the tools Snoopy~\cite{SnoopyTool}, MARCIE~\cite{MARCIETool} and Spike~\cite{SpikeTool}. It proved to be generally faster than the method presented in~\cite{PatternPaper}. 

In~\cite{MCCUnfolder} (MCC) Dal Zilio describes a method which he calls \textit{stable places}. A stable place is a place that never changes from the initial marking, i.e. every time a token is consumed from this place an equivalent token is added to the place. For a place to be stable it has to hold that for each transition the place is connected to, it is connected by both an input and output arc that have equivalent arc expressions. As such, it is only a syntactical check, meaning no further analysis is done. This method is especially efficient on the net BART from the Model Checking Contest~\cite{mcc:2020}. However, this method is not very general and does not find places that deviate even a little from the initial marking. The color approximation method is a more general form of the stable places and is able to capture these deviations from the initial marking. In~\cite{MCCUnfolder} an additional method called \textit{Component Analysis} is presented where it is detected that a net consists of a number of copies of the same component. MCC is used in the TINA toolchain~\cite{TINAtool} and to our knowledge in the latest release of the LoLA tool~\cite{LoLA2}. 

GreatSPN~\cite{GSPNPaper} is another tool for unfolding CPNs, however in~\cite{MCCUnfolder} it is demonstrated that MCC was able to greatly outperform GreatSPN and as such we omit GreatSPN from later experiments.

ITS-Tools~\cite{ITSToolPaper} has an integrated unfolding engine. The tool uses a technique we refer to as \textit{variable symmetry identification}, in which it is analyzed whether variables $x$ and $y$ are actually permutable in a binding. This allows for invalidation of bindings that are equivalent by constraining $x \leq y$.  Furthermore, they use stable places during the binding and they apply analysis to choose the binding order of parameters to simplify false guards as soon as possible. 
After unfolding ITS-Tools applies some post-unfolding reductions that removes orphan places and transitions and removes behaviourally equivalent transitions should they make them~\cite{YannCorrespondence}. 

In \cite{YannSymmetryDetection} Thierry-Mieg et al. present a technique for automatic detection of symmetries in high level Petri nets used to construct symbolic reachability graphs in the GreapSPN tool. This detection of symmetries is very reminiscent of the color quotienting method presented in this paper, although the color quotienting method is used for unfolding the colored Petri net instead of symbolic model checking.

In~\cite{KlostergaardThesis} Klostergaard presents the unfolding method implemented in \textit{verifypn} revision 226 (untimed engine of TAPAAL~\cite{TAPAALTool, verifypnPaper}), which is the base of our implementation. The implementation is efficient, but since it is implemented as the naive approach mentioned earlier, there are several nets which it cannot unfold such as BART.

Both the color quotienting method and the color approximation method are advanced static analyses techniques and all of the above mentioned techniques, except symmetric variables and component analysis, are captured by color approximation and color quotienting.

\subsection{Bibliographical Remark}
Parts of this thesis are inspired or derived from the work in our 9th semester project~\cite{ninthsemester}. Specifically, the Abstract and Section~\ref{sec:Introduction} are modified and extended versions from the previous work where especially the related work has been extended to cover more related tools. Section \ref{sec:Preliminaries} has been modified s.t. we instead define bisimulation and define isomorphism as a special case of bisimulation. Section \ref{Sec:IntegerCPN} uses the same syntax and semantics as described in~\cite{ninthsemester} but is described more informally in this work. Section \ref{Sec:ColorApprox} is a revised and improved version of the main contribution in~\cite{ninthsemester}. Specifically, we have updated the color expansion to be a function instead of a transition relation, in order to use fixed point theory. The rest of the section is adjusted accordingly. Furthermore, we optimize the color approximation implementation presented in~\cite{ninthsemester}. Lastly, Section~\ref{sec:FutureWork} includes similar future work as in the previous work, but we extend it to consider new data structures and the new methods presented in this project. 


==> Introduction/abstract.tex <==
\begin{abstract}
 Colored Petri nets offer a compact and user friendly representation of traditional Petri nets also known as P/T nets. Colored Petri nets with finite color ranges can be unfolded into traditional P/T nets. However, this unfolding may produce exponentially larger P/T nets. We present two novel formal techniques based on static analyses for reducing the size of unfolded colored Petri nets. The first method identifies colors that behave equivalent in the colored Petri net and groups them into equivalence classes representing the colors, producing a smaller quotiented colored Petri net. The second method analyses which colors can ever exist in any place and excludes colors that can never be present in a given place. Both methods show great promise individually, but even more when combined. The combined method is able to reduce the size of multiple colored Petri nets from the Model Checking Contest compared to state of the art unfolders MCC, Spike and ITS-Tools, while still remaining competitive in terms of unfolding time. Lastly, we show the effect of the smaller unfolded nets by verifying queries from the 2020 Model Checking Contest using the unfolded nets from each tool.
\end{abstract}

==> Tables/ConstantSizesTable.tex <==

\begin{table}[]
\centering
\begin{tabular}{l|llll}
     & A+B & ITS & MCC & Spike \\ \hline
AirplaneLD-COL-0010        & 55      & 145     & 177     & 177       \\
AirplaneLD-COL-0020        & 55      & 265     & 327     & 327       \\
AirplaneLD-COL-0050        & 55      & 625     & 777     & 777       \\
AirplaneLD-COL-0100        & 55      & 1225    & 1527    & 1527      \\
AirplaneLD-COL-0200        & 55      & 2425    & 3027    & 3027      \\
AirplaneLD-COL-0500        & 55      & 6025    & 7527    & 7527      \\
AirplaneLD-COL-1000        & 55      & 12025   & 15027   & 15027     \\
AirplaneLD-COL-2000        & 55      & 24025   & 30027   & 30027     \\
AirplaneLD-COL-4000        & 55      & 48025   & 60027   & 60027     \\
BART-COL-002               & 447     & 668     & 1410    & -         \\
BART-COL-005               & 447     & 1670    & 3117    & -         \\
BART-COL-010               & 447     & 3340    & 5962    & -         \\
BART-COL-020               & 447     & 6680    & 11652   & -         \\
BART-COL-030               & 447     & 12509   & 17342   & -         \\
BART-COL-040               & 447     & 13360   & 23032   & -         \\
BART-COL-050               & 447     & 16700   & 28722   & -         \\
BART-COL-060               & 447     & 20040   & 34412   & -         \\
DrinkVendingMachine-COL-02 & 22      & 76      & 96      & 96        \\
DrinkVendingMachine-COL-10 & 22      & 28780   & 111280  & 111280    \\
DrinkVendingMachine-COL-16 & 22      & 248352  & 1118752 & 1118752   \\
DrinkVendingMachine-COL-24 & 22      & 1685232 & 8309232 & -         \\
DrinkVendingMachine-COL-48 & 22      & -       & -       & -         \\
DrinkVendingMachine-COL-76 & 22      & -       & -       & -         \\
DrinkVendingMachine-COL-98 & 22      & -       & -       & -         \\
Referendum-COL-0010        & 7       & 52      & 52      & 52        \\
Referendum-COL-0015        & 7       & 77      & 77      & 77        \\
Referendum-COL-0020        & 7       & 102     & 102     & 102       \\
Referendum-COL-0050        & 7       & 252     & 252     & 252       \\
Referendum-COL-0100        & 7       & 502     & 502     & 502       \\
Referendum-COL-0200        & 7       & 1002    & 1002    & 1002      \\
Referendum-COL-0500        & 7       & 2502    & 2502    & 2502      \\
Referendum-COL-1000        & 7       & 5002    & 5002    & 5002     
\end{tabular}
\caption{Nets with constant size scaling. A '-' indicates that the net was not unfolded by the tool}
\label{tab:constantSizeScaling}
\end{table}

==> Tables/EngineOptionTable.tex <==

\begin{table}[h]
\centering
\begin{tabular}{l|ccccccc}
 &
  \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Arc \\ Analysis\end{tabular}} &
  \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Guard \\ Analysis\end{tabular}} &
  \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Stable \\ places\end{tabular}} &
  \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Component\\ Analysis\end{tabular}} &
  \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Colorset \\ Reduction\end{tabular}} &
  \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Symbolic \\ Colorsets\end{tabular}} \\\hline
Old verifypn                                                                 &$\div$        &$\div$        &$\div$        &$\div$        &$\div$     & $\div$      \\
Snoopy \tablefootnote{From 2012 paper\cite{PatternPaper}}                           &\checkmark&\checkmark&$\div$        &$\div$    &$\div$ & $\div$        \\
MCC                                                                            &\checkmark&\checkmark&\checkmark&\checkmark &  $\div$ & $\div$         \\
New verifypn &\checkmark&\checkmark&\checkmark&$\div$  & \checkmark & $\checkmark$
\end{tabular}
\caption{Some engines and their attributes}
\label{tab:EngineOptionTable}
\end{table}
